The Atiyah--Hitchin bracket for the cubic Nonlinear Schrodinger equation. IV. the scattering potentials

This is the last in a series of four papers on Poisson formalism for the cubic nonlinear Schrodinger equation with repulsive nonlinearity. In this paper we consider scattering potentials.

==> 00README.XXX.tex <==
nohypertex
